Robust Federated Learning Mitigates Client-side Training Data Distribution Inference Attacks

Recent studies have revealed that federated learning (FL), once considered secure due to clients not sharing their private data with the server, is vulnerable to attacks such as client-side training data distribution inference, where a malicious client can recreate the victim's data. While various countermeasures exist, they are not practical, often assuming server access to some training data or knowledge of label distribution before the attack. In this work, we bridge the gap by proposing InferGuard, a novel Byzantine-robust aggregation rule aimed at defending against client-side training data distribution inference attacks. In our proposed InferGuard, the server first calculates the coordinate-wise median of all the model updates it receives. A client's model update is considered malicious if it significantly deviates from the computed median update. We conduct a thorough evaluation of our proposed InferGuard on five benchmark datasets and perform a comparison with ten baseline methods. The results of our experiments indicate that our defense mechanism is highly effective in protecting against client-side training data distribution inference attacks, even against strong adaptive attacks. Furthermore, our method substantially outperforms the baseline methods in various practical FL scenarios.

==> macros.tex <==

%
% The name of this file is ``macros.tex''
%

%
% TEX defaults
%
%
% frame 6.5 * 9
\textwidth 6.5in
\textheight 9in

% left/right margins
\oddsidemargin 0pt
\evensidemargin 0pt
\marginparwidth 1in
\marginparsep 0pt

% top margin
\topmargin -25pt
\headheight 10pt
\headsep 30pt
% \topskip 0pt

% foot margin
%\footheight 0pt
\footskip 27pt


% macros for commonly used special fonts
\newcommand{\IE}{{\it i.e.,}\ }
\newcommand{\EG}{{\it e.g.,}\ }
% single/double spacing
%\newcommand{\SS}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\DS}{\renewcommand{\baselinestretch}{1.6}\large\normalsize}
% reduce the space between lines
\newcommand{\Tight}{\renewcommand{\baselinestretch}{0.9}\large\normalsize}
\newcommand{\HalfTight}{\renewcommand{\baselinestretch}{0.95}\large\normalsize}
\newcommand{\MinorTight}{\renewcommand{\baselinestretch}{0.975}\large\normalsize}
% Page title (primarily for foils)
% (this was called \HH}
\newcommand{\PageTitle}[1]{{\newpage \begin{center}{\LARGE {\bf {#1}} } \end{center} } }

% remove spaces around section headers
%\newcommand{\Section}[1]{\vspace{-3ex}\section{#1}\vspace{-2ex}}
\newcommand{\Subsection}[1]{\vspace{-2ex}\subsection{#1}\vspace{-1ex}}
\newcommand{\Subsubsection}[1]{\vspace{-2ex}\subsubsection{#1}\vspace{-1ex}}

% go forward n lines (negative for backward move)
\newcommand{\VLine}[1]{\vspace{#1ex}}
% itemize and enumerate without spaces around/between items
\newenvironment{TightItem}{\vspace{-2ex}\begin{itemize}
  \setlength{\itemsep}{-0ex}}{\end{itemize}\vspace{-1ex}}
\newenvironment{TightEnum}{\vspace{-2ex}\begin{enumerate}
  \setlength{\itemsep}{-0ex}}{\end{enumerate}\vspace{-1ex}}
\newenvironment{TightDesc}{\vspace{-1ex}\begin{description}
  \setlength{\itemsep}{-0ex}}{\end{description}\vspace{-1ex}}
% set the page number (to the first argument)
\newcommand{\SetPageNo}[1]{\countdef\pageno=0 \pageno=#1}
% things to do
\newenvironment{Todo}{\begin{large}\begin{bf}********** things to do
    ********** \\}{\\ **********\end{bf}\end{large}}
% for discussion
\newenvironment{Discuss}{\begin{large}\begin{em}**********
    things to be discussed ********** \\}{\\ **********\end{em}\end{large}}
% set the paragraph identation and separation


% the foil environment
\newenvironment{Foil}{\begin{document}\begin{LARGE}\begin{sf}
    }{\end{sf}\end{LARGE}\end{document}}
    % NOTE: ``}'' must be in the 2nd line
% foil page title
\newcommand{\Title}[1]{\newpage \center{\huge {\sf #1}} \flushleft
    \vspace{1ex}}

% set the paragraph identation and separation
\parindent 0.2in
\setlength{\parskip}{1ex}

% set text width
\textwidth = 6.75in

% set the formula separation
\setlength{\topsep}{0in}

% set indentation for formulas:
% \setlength{\mathindent}{3ex}

% set left margin
\setlength{\oddsidemargin}{-.1in}



